SmartExchange: Trading Higher-cost Memory Storage/Access for Lower-cost Computation

We present SmartExchange, an algorithm-hardware co-design framework to trade higher-cost memory storage/access for lower-cost computation, for energy-efficient inference of deep neural networks (DNNs). We develop a novel algorithm to enforce a specially favorable DNN weight structure, where each layerwise weight matrix can be stored as the product of a small basis matrix and a large sparse coefficient matrix whose non-zero elements are all power-of-2. To our best knowledge, this algorithm is the first formulation that integrates three mainstream model compression ideas: sparsification or pruning, decomposition, and quantization, into one unified framework. The resulting sparse and readily-quantized DNN thus enjoys greatly reduced energy consumption in data movement as well as weight storage. On top of that, we further design a dedicated accelerator to fully utilize the SmartExchange-enforced weights to improve both energy efficiency and latency performance. Extensive experiments show that 1) on the algorithm level, SmartExchange outperforms state-of-the-art compression techniques, including merely sparsification or pruning, decomposition, and quantization, in various ablation studies based on nine DNN models and four datasets; and 2) on the hardware level, the proposed SmartExchange based accelerator can improve the energy efficiency by up to 6.7$\times$ and the speedup by up to 19.2$\times$ over four state-of-the-art DNN accelerators, when benchmarked on seven DNN models (including four standard DNNs, two compact DNN models, and one segmentation model) and three datasets.

==> tex/Framework_for_Energy_and_Performance_Analysis.tex <==
\vspace{-1em}
\section{Proposed Analytical Models}\label{sec:Framework}

This section introduces another contribution of this paper, which is that we propose an analytical modelling framework to accurately predict DNN accelerators' inference energy cost, latency, and throughput when employing various dataflows and hardware configurations. Specifically, Section~\ref{subsec:design_space} presents the employed approach of describing DNN accelerators' design space, Section~\ref{subsec:framework} provides the details of our performance models and shows how these models can be used for design optimization (e.g., finding the optimal dataflow), and Section~\ref{subsec:validation} describes the model validation performed by comparing our models' predicted performance with actual chip-measured ones from a state-of-the art DNN accelerator \cite{chen2017eyeriss} under varied design configurations.

\ul{The advantages of our proposed models} are that they \emph{(i)} match well with actual chip measurements ($\le$ 18\%); \emph{(ii)} are analytical and intuitive (directly tie to the DNN model and accelerator parameters), facilitating their ease of use for time-efficient design space exploration and optimization; and \emph{(iii)} are programmer friendly and compatible with commonly used DNN frameworks (e.g., Pytorch \cite{paszke2017automatic}, Caffe \cite{jia2014caffe}, and Tensorflow \cite{tensorflow2015-whitepaper}) thanks to their employed generic nested for-loop description of DNN accelerators' design space.

\vspace{-0.5em}
\subsection{Design Space Description}\label{subsec:design_space}
%   \vspace{-1em}
   
\begin{figure}[h]
   \vspace{-2em}
  \begin{algorithm}[H]
    \begin{algorithmic}[1]
    \Statex
    \State{\hspace{0pt}  {{\color{orange}// DRAM level}} }
    \State{\hspace{0pt}for ($m_3$=0; $m_3$<$M_3$; $m_3$++) \{}
    \State{\hspace{10pt}  {{\color{orange}// Global buffer level}} }
    \State{\hspace{10pt} {\color{blue} \Rightarrow{$GB_{input}$ refresh} }}
    \State{\hspace{10pt}for ($m_2$=0; $m_2$<$M_2$; $m_2$++) \{}
    \State{\hspace{20pt} {\color{blue}\Rightarrow{$GB_{weight}$ refresh} }}
    \State{\hspace{20pt}for ($e_2$=0; $e_2$<$E_2$; $e_2$++) \{}
    \State{\hspace{30pt}for ($f_2$=0; $f_2$<$F_2$; $f_2$++) \{}
    \State{\hspace{40pt} {\color{blue}\Rightarrow{ $GB_{output}$ refresh} }}
    \State{\hspace{40pt} {{\color{orange}// NoC level}} }
    \State{\hspace{40pt}parallel-for ($e_1$=0; $e_1$<$E_1$; $e_1$++) \{}
    \State{\hspace{40pt}parallel-for ($f_1$=0; $f_1$<$F_1$; $f_1$++) \{}
    \State{\hspace{50pt} {{\color{orange}// RF level}} }
    \State{\hspace{50pt} {\color{blue}\Rightarrow{$RF_{input}$ refresh, $RF_{weight}$ refresh}}}
    \State{\hspace{50pt}for ($c_0$=0; $c_0$< $C_0$; $c_0$++) \{}
    \State{\hspace{60pt}for ($r_0$=0; $r_0$<$R_0$; $r_0$++) \{}
    \State{\hspace{70pt}for ($s_0$=0; $s_0$<$S_0$; $s_0$++) \{}
    \State{\hspace{80pt}MAC operation}
    \State{\hspace{80pt} {\color{blue}\Rightarrow{ $RF_{output}$ refresh} \}\}\}\}\}\}\}\}\}}
%\State{\hspace{70pt} O += W $\times$ I}
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
  \caption{\textbf{An example of using a nested for-loop representation to describe the design space of DNN accelerators, considering a CONV layer.}}
  \label{fig:loop1}
   \vspace{-1.0em}
\end{figure}

For modeling the DNN accelerators' performance given their large design space, one critical question is \textit{how to describe the whole design space, i.e., cover all possible design choices, in a way that is easy to understand and to follow?} For ease of use and better visualization, we extend the nested for-loop description of row stationary in~\cite{eyeriss} to describe the design space as shown in Fig.~\ref{fig:loop1}. Specifically, we employ \ul{(i) the primitive, \textit{for}}, to describe the temporal operations of each PE as well as the temporal data tiling and mapping operations at the DRAM, GB and RF levels; and \ul{(ii) the primitive, \textit{parallel-for}}, to describe the spatial data tiling and mapping operations at the NoC level (i.e., in the PE array). Without loss of generality, we consider four levels of memory hierarchy, i.e., off-chip DRAM, on-chip GB, NoC in the PE array, and RF within the PEs. The design space of DNN accelerators mainly includes two aspects: hardware design configurations and dataflows.

\textbf{Hardware configurations} which can be described using a set of architecture-dependent hardware parameters and technology-dependent design parameters. In particular, the architecture-dependent hardware parameters includes PE array architectures (e.g., spatial array, systolic array, and adder tree), number of PEs, NoC design (e.g., unicast, multicast, or broadcast), memory hierarchies, and the storage capacity and communication bandwidth of each memory hierarchy; the technology-dependent design parameters includes unit energy/delay costs of a MAC operation and memory accesses to various memory hierarchies, and the clock frequency.

\textbf{Dataflows} which are to describe how a DNN algorithm is temporally and spatially scheduled to be executed in an accelerator. Specifically, a dataflow answers the following questions: \emph{(i)} \textit{how to map and schedule the computations in the PE array and within each PE}?; and \emph{(ii)} \textit{what are the loop ordering and tiling factors on the DRAM and global buffer levels}? The former corresponds to the design choice of holding a certain type of data locally in the PE once it is fetched from the memories, e.g., row, weight, or output stationary. The latter can be described using three groups of parameters as defined below in the context of the example in Fig.~\ref{fig:loop1}, which shows an output stationary dataflow~\cite{eyeriss} for the proposed \textit{SmartExchange} accelerator (see Fig.~\ref{fig:overview_PE}): \ul{Loop ordering factors} for the nested twenty-four loops associated with the six dimensions of the 3D convolution operation in a CONV layer (see Eq. (\ref{eq:CONV})) and the four considered memory hierarchies (i.e., DRAM, GB, NoC, and RF); \ul{Loop tiling factors} for the nested twenty-four loops associated with the six dimensions of the 3D convolution operation in a CONV layer and the four considered memory hierarchies; and \ul{Data access locations} where (in which of the six nested for-loops that describes the 3D CONV layer operations as shown in Eq. (\ref{eq:CONV})) we refresh the on-chip GB and in-PE RFs for the input activations, output activations, and weights. 

\vspace{-0.5em}
\subsection{The Proposed Modelling Framework}\label{subsec:framework}
\vspace{-1em}
\subsubsection{Overview}
\vspace{-0.3em}
\begin{figure}[h]
   \vspace{-0.5em}
    \centerline{\includegraphics[width=75mm]{fig/analytical_models.png}}
       \vspace{-0.5em}
    \caption{\textbf{A high-level view of the proposed modelling framework} }
    \label{fig:df}
    \vspace{-2em}
\end{figure}

Fig.~\ref{fig:df} shows a high-level view of the proposed model framework, which accepts DNN models (e.g., number of layers, layer structure, precision, etc.), hardware configuration parameters (e.g., memory hierarchy, number of PEs, NoC design, etc.), dataflows (e.g., row/weight/output stationary, loop tiling/ordering factors, etc.), and technology-dependent unit costs (e.g., unit energy/delay cost of a MAC operation and memory accesses to various memory hierarchies), and then outputs the estimated energy consumption, latency, and throughput when executing the DNN in the target accelerator defined by the given hardware configuration parameters. 

The proposed analytical models can be used to \emph{(i)} validate DNN accelerator techniques without the time- and cost-consuming necessity of designing the accelerator chips, and \emph{(ii)} perform time-efficient design space exploration and optimization. For example, given a hardware configuration and DNN model, the search for the optimal dataflow $DF_{alg_{\veryshortarrow}hw}^*$, that minimizes the energy cost, can be formulated as:

\vspace{-1.5em}
\begin{equation}
    \begin{aligned}
% \begin{align}
       DF_{alg_{\veryshortarrow} hw}^* = 
        &\underset{DF_{alg_{\veryshortarrow} hw}}{\mathrm{arg}}{ \mathrm{min}}\,\,E_{DNN}(\textbf{P}_{DNN}, DF_{alg_{\veryshortarrow} hw}, \textbf{e}_{tech}, \textbf{P}_{hw}})\\
        %&\mathrm{subject\ to} \quad Th_{DNN} \ge Th_{min}, \,\,L_{DNN} \le L_{max}
        &\mathrm{s.t.} \quad Th_{DNN} \ge Th_{min}, \,\,L_{DNN} \le L_{max}
        \label{eq:opt-df}
% \end{align}
    \end{aligned}
    \vspace{-1em}
\end{equation}
where $\textbf{P}_{DNN}$, $DF_{alg_{\veryshortarrow} hw}$, and $\textbf{P}_{hw}$ denote the model parameters that define a DNN, dataflow, and hardware design configuration parameters that define the accelerator, respectively, $E_{DNN}$, $Th_{DNN}$, and $L_{DNN}$ denote the energy consumption, throughput, and latency of operating the DNN in the accelerator, respectively, and technology-dependent unit costs are denoted by $\textbf{e}_{tech}$. The performance limits $Th_{min}$ and $L_{max}$ denote the minimum inference throughput and maximum inference latency that are acceptable to and imposed by the target application. Our models can analytically formulate $E_{DNN}$ as a function of the model parameters (i.e., $\textbf{P}_{DNN}$) and accelerator design parameters (e.g., $DF_{alg_{\veryshortarrow} HW}$ and $\textbf{P}_{hw}$). 

\vspace{-0.5em}
\subsubsection {The Analytical Performance Models}\label{subsec:perf_model}

This subsection introduces our proposed analytical models for both DNN accelerators' energy and latency.

\textbf{Energy Models}. 
The energy of DNN accelerators include both computational ($E_{comp}$) and data movement ($E_{DM}$) costs, i.e., $E_{DNN} =  E_{comp} + E_{DM}$, where $E_{comp} = N_{MAC}\times e_{MAC}$ with $N_{MAC}$ denoting the total number of MACs in the DNN. Similarly, 
% $E_{DM}$ can be written as follows:
the data movement cost can be calculated by multiplying the unit energy cost per access ($e_{DM_{i,j}}, j \in \{I, O, W\}$)  with the total number of accesses ($N_{DM_{i,j}}, j \in \{I, O, W\}$) to the $i$-th memory hierarchy (e.g., GB and RF) using the $j$-th type of data (i.e., inputs ($I$), outputs ($O$), and weights ($W$)):  
\vspace{-0.3em}
\begin{align}
% \vspace{-3em}
\label{eq:DM}
    E_{DM} = \sum_{i \in S_{Memory}}\sum_{j \in \{I, O, W\}} N_{DM_{i,j}}, \times e_{DM_{i,j}}
\end{align}
\vspace{-0.7em}
\\where $S_{Memory} = \{DRAM \shortarrow GB, GB \shortarrow NoC, NoC \shortarrow RF, RF \shortarrow PE \}$ for inputs/weights; and $S_{Memory} = \{DRAM \leftrightarrow GB, GB \leftrightarrow NoC, NoC \leftrightarrow RF, RF \leftrightarrow MAC\}$ for outputs.
 
\textbf{The key challenge is to obtain $N_{DM_{i,j}}$} for various memory hierarchies and data types when using different DNN models, hardware configurations, and dataflows. We suggest that $N_{DM_{i,j}}$ can be calculated as the product between the $j$-th data volume ($V_{ref_{i,j}}$)  involved in each refresh and the total number of such refreshes ($N_{ref_{i,j}}$) for the $i$-th memory, i.e.,  
\vspace{-0.6em}
\begin{align}
    N_{DM_{i,j}} = N_{ref_{i,j}} \times V_{ref_{i,j}}
\end{align}
\vspace{-1.5em}
\\To obtain $N_{ref_{i,j}}$ and $V_{ref_{i,j}}$, \textbf{we propose an intuitive methodology}: we first \ul{\textbf{(i)}} choose a refresh location, which can be straightforwardly decided once the dataflow is known, in the nested for-loops (see Fig. \ref{fig:loop1}) for a given  data type; \ul{\textbf{(ii)}} $N_{ref_{i,j}}$ is equal to the product of all the loop bounds in the for-loops \textbf{below} the refresh location and associated with this type of data; and \ul{\textbf{(iii)}} $V_{ref_{i,j}}$ is equal to the product of all the loop bounds in the for-loops \textbf{above} the refresh location and associated with this type data. Once $N_{ref_{i,j}}$ and $V_{ref_{i,j}}$ are obtained, the energy can be calculated as: 
\vspace{-0.6em}
\begin{align}
    E_{DRAM} &= \sum_{j \in \{I,O,W\}} N_{ref_{GB,j}} \times V_{ref_{GB,j}} \times e_{DM_{GB,j}}\\
    E_{GB} &= \sum_{j \in \{I,O,W\}} N_{ref_{RF,j}} \times V_{ref_{RF,j}}\times \frac{N_{PE}}{M_j} \times e_{DM_{NoC,j}}\\
    E_{NoC} &= \sum_{j \in \{I,O,W\}}N_{ref_{RF,j}} \timesV_{ref_{RF,j}} \times N_{PE}\times e_{DM_{NoC,j}}\\
    E_{RF} &= \sum_{j \in \{I,O,W\}} N_{MAC} \times e_{DM_{RF,j}}
\end{align}
\vspace{-1em}
\\where $N_{PE}$ is the number of active PEs and $M_j$ is the number of PEs that share the same data.

\textbf{Latency Models}. Similarly, the latency of DNN accelerators can be formulated as:
\vspace{-0.6em}
\begin{align}
    L = L_{setup} + \max \{L_{DRAM}, L_{GB}, L_{comp}\}
\end{align}
\vspace{-1.6em}
\\where $L_{comp}$ denotes the computation latency, $L_{DRAM}$ denotes the latency of accessing the DRAM from the GB, $L_{GB}$ denotes the latency of accessing the GB from an RF in the PEs, and $L_{setup}$ denotes the setup latency to load the first set of the weights and inputs. Adopting $N_{bit}^j$-bit precision for inputs/outputs/weights is $N_{bit}^j$, $j \in \{I,O,W\}$, we have:
\vspace{-5pt}
\begin{align}
    L_{comp} &= N_{MAC} \times t_{comp}\\
    L_{DRAM} &= \max_{j \in \{I,O,W\}} N_{ref_{GB,j}} \times \frac{V_{ref_{GB,j}}\times N_{bit}^j}{\min\{BW^j_{GB}, BW_{DRAM}\}}\\
    L_{GB} &= \max_{j \in \{I,O,W\}} N_{ref_{RF,j}} \times \frac{N_{ref_{RF,j}}\times N_{bit}^j\times N_{PE}}{BW^j_{GB}}\\
    L_{setup} &= \max (L^{'}_{DRAM}, L^{'}_{GB})\\
    L^{'}_{DRAM} &=\max_{j \in \{I,W\}} \frac{V_{ref_{GB,j}}\times N_{bit}^j}{\min\{BW_{j,{GB}}, BW_{DRAM}\}}\\
    L^{'}_{GB} &=\max_{j \in \{I,W\}} \frac{N_{ref_{RF,j}}\times N_{bit}^j}{\min\{BW_{j,{RF}}, BW_{j,{GB}}\}}
\end{align}
\vspace{-0.6em}
\\where $BW^j_{i}$ is the memory bandwidth for the $i$-th memory hierarchy for the data type $j \in \{I,O,W\}$.
% \begin{figure}[!b]
% \captionsetup[subfigure]{labelformat=empty}
%     \centering
%     \centerline{\includegraphics[width=80mm]{fig/energy_breakdown_new_mark.png}}
%     \vspace{-1em}
%     \caption{\textbf{Comparison on the energy breakdown from Eyeriss~\cite{chen2017eyeriss} and our models, for the CONV1 (left) and CONV5 (right) of AlexNet\cite{NIPS2012_4824}.} \todor{not update}}
%   \vspace{-1em}
%     \label{fig:val_1}
% \end{figure}

\begin{table}%[!b]
\centering
\vspace{3mm}
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}c | cc c cc c cc c cc@{}}\toprule
\multirow{2}{*}{Layer}& \multicolumn{2}{c}{comp.} & \phantom{x}& \multicolumn{2}{c}{RF} & \phantom{x}& \multicolumn{2}{c}{NoC} & \phantom{x}& \multicolumn{2}{c}{GB}\\ 
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
& Meas. & Pred. && Meas. & Pred. && Meas. & Pred. && Meas. & Pred.  \\ 
\midrule
\multirow{1}{*}{CONV1}
$ $ & 16.7\% & 18.7\% && 79.6\% & 74.4\% && 1.7\% & 4.8\% && 2.0\% & 2.0\%\\
% \midrule
\multirow{1}{*}{\textbf{$\Delta$}}
$ $ & \multicolumn{2}{c}{\textbf{2.08\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-5.15\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{3.10\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-0.03\%}}\\
\midrule
\multirow{1}{*}{CONV5}
$ $ & 7.3\% & 7.5\% && 80.3\% & 79.1\% && 5.3\% & 7.0\% && 7.0\% & 6.3\%\\
% \midrule
\multirow{1}{*}{\textbf{$\Delta$}}
$ $ & \multicolumn{2}{c}{\textbf{0.26\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-1.16\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{1.64\%}} & \phantom{x}& \multicolumn{2}{c}{\textbf{-0.74\%}}\\
\bottomrule
\end{tabular}
\vspace{-0.3em}
\caption{\textbf{The energy breakdown from Eyeriss~\cite{chen2017eyeriss} and our models, for the CONV1 and CONV5 of AlexNet\cite{NIPS2012_4824}.}}
\label{fig:val_1}
\vspace{-2.2em}
\end{table}

\vspace{-0.4em}
\subsection{Model Validation}\label{subsec:validation}
\vspace{-0.3em}
% \begin{table*}[htbp]
% \centering
% \vspace{-1em}
% {%\footnotesize
% \scriptsize
% \small
%     \label{tab:MultiBackboneMultiDataset}
%     \begin{tabular}{@{}C{2cm}C{3cm}C{3cm}C{3cm}C{2cm}C{2cm}@{}} \toprule
%     Prediction Error  & Latency & PE utilization & Energy Breakdown & \# of DRAM accesses & \# of GB accesses\\ \midrule
%     ASIC Measurement\cite{eyeriss} & -15.5\% \sim-4.1\% & - & -10.5\% \sim +12.5\% & -11.1\% \sim -2.2\% & -17.7\% \sim +0.7\%\\ 
%     \midrule
%     FPGA Synthesis\cite{hao2019fpga} & -16.8\% \sim -0.3\% & -13.4\% \sim -1.4\% & - & - & -\\
%     % \midrule
%     % ASIC Synthesis & - & - & - & - & -\\
%     \bottomrule
%     \end{tabular}
%     % \end{adjustbox}
% }
% \vspace{-0.5em}
% \caption{Analytical model validation against state-of-the-art DNN accelerators.}
% \label{table:val}
% \end{table*}

We validate our proposed analytical models by comparing our modeles' predicted performance with actual chip measured ones in~\cite{eyeriss}, FPGA implementation results in~\cite{hao2019fpga}, and synthesis results based on a commercial technology, under the same experiment settings (e.g., unit energy, clock frequency, DNN model, architecture design and dataflow, etc). 

\textbf{Validation against Chip Measurements.} For this set of experiments, we compare our models' predicted performance with Eyeriss' chip-measured results using their normalized unit energy~\cite{eyeriss}. First, Table~\ref{fig:val_1} compares the \ul{energy breakdown} of AlexNet\cite{NIPS2012_4824}'s first and fifth CONV layers, showing that the maximum difference is 5.15\% and 1.64\%, respectively. 
% The difference in terms of the NoC energy is relatively larger because our models' employed unit energy of NoC considers the average wire length between PEs when PE utilization is 100\%, whereas actual PE utilization depends on DNN model structures and the actual PE array size. For better prediction accuracy, we can further fine tune the unit energy of NoC for the employed DNN models and hardware design. 
Second, Fig.~\ref{fig:val_2} compares \ul{the number of DRAM/GB accesses}. The difference between the predicted number of DRAM accesses and Eyeriss's measured results is between 2.18\% and 12.10\%, while the difference in terms of GB accesses is between -0.70\% and 17.66\%. Our models' predicted DRAM access number is smaller than that of Eyeriss because the RLC overhead of sparse activations depends on the input images and we lack the information about which set of images were used in Eyeriss's measurements. Additionally, Fig.~\ref{fig:val_2} shows that the difference between the predicted number of GB accesses and Eyeriss's results is less than 5\% except for the CONV1 layer where the relative larger prediction error is caused by its larger stride, which is 4. Specifically, a larger stride leads to less utilization of inputs fetched from the GB, whereas our current models consider the generic case where stride is 1 as it is more often seen in recent DNN models. For better prediction accuracy, the models can be adjusted to consider cases with strides of larger than 1. 

% more frequent occurrence of cases where the data accesses from the GB and the computation can not be fully pipelined, whereas our current models consider only the generic case where this pipeline is mostly effective for generality. 

Third, Fig.~\ref{fig:latency} compares the \ul{latency} of executing AlexNet\cite{NIPS2012_4824}'s five CONV layers, and shows that the predicted and Eyeriss's ones differ $\le$ 15.51\%. The predicted latency is smaller than the measured one because our models do not consider the corner cycles when the memory accesses and computation can not be fully pipelined where processing stalls occur. Finally, the predicted \ul{throughput} of executing AlexNet is 46.0 GOPS while the one measured by Eyeriss is 51.6 GOPS, showing a prediction error of $\le$11\%. 


\textbf{Validation against FPGA Implementation.} We compare our models' predicted latency with FPGA measured ones under the same DNN model and hardware configurations~\cite{zhang2019skynet}. Specifically, for the FPGA one we use the open source implementation of the award winner~\cite{zhang2019skynet} in a state-of-the-art design contest~\cite{dac-contest}. Fig.~\ref{fig:val_fpga} shows that our models' predicted latency differs by the FPGA-synthesized ones by $\le$ 16.84\%. Note that in FPGA implementations the GB can be partitioned into smaller chunks to be accessed simultaneously for increasing the parallelism and minimizing the latency. Our current models do not include the overhead of this partition, which is larger when the GB is partitioned into more chunks for layers with larger size, leading to a larger prediction error for the CONV4/CONV5/CONV6 layers in Fig. ~\ref{fig:val_fpga}.

% \hl{We validate our proposed analytical models against XX state-of-the-art architectures including ASIC-based}~\cite{eyeriss} and FPGA-based~\cite{hao2019fpga} accelerators as shown in Table~\ref{table:val}. \hl{We compare the predicted performance with the ground truth obtained from the real measurement or the synthesis results, and we can observe a prediction error from -17.7\% to 12.5\% when adopting the same experiment settings as the ground truth, e.g. unit energy values, clock frequency, NN model, architecture design and dataflow.

% We have three sets of experiment targeting on different architectures. First, for the validation experiment with the Eyeriss}~\cite{eyeriss} \hl{architecture, we use row stationary dataflow and the five convolution layers of AlexNet to compare the energy breakdown (including energy for DRAM, GB, RF and computation on CONV1 and CONV5 of AlexNet), latency, DRAM accesses, and GB accesses under 200MHz clock frequency. Second, for the experiment with the FPGA accelerator from}~\cite{hao2019fpga}, \hl{we use weight stationary dataflow (with different tiling factors) and a compact NN model} ~\cite{zhang2019skynet} from the winner of the design contest~\cite{dac-contest} to compare the latency and PE utilization under the 100MHz clock frequency. \hl{Third, for the ASIC synthesis XX}

% \hl{The prediction error for latency on FPGA increases as we increase the tiled array size, since we assume each 2D array of data can be fully partitioned during the data transfer; however, the latency overhead for the array partition is not negligible when the array size is above a threshold. The prediction error for PE utilization on FPGA comes from an imprecise prediction for the ReLU layer.}


% To validate the proposed analytical models as described in Section \ref{subsec:perf_model}, we compare the performance predicted by our models with chip-measured performance of Eyeriss~\cite{chen2017eyeriss} when using the same \hl{unit energy cost}~\cite{eyeriss}, hardware parameters, DNN models, dataflow, etc. First, Fig.~\ref{fig:val_1} shows that the maximum differences between the models' predicted relative energy breakdown of AlexNet\cite{NIPS2012_4824}'s first and fifth CONV layers and Eyeriss's measured results are 10.3\% and 8.9\%, respectively. \todor{update Fig.~\ref{fig:val_1}}. \hl{The largest relative predicted error lies in NoC because the the NoC unit energy cost is gotten from long distance.} 
% Second, we compare the number of DRAM accesses and the number of GB accesses in Fig.~\ref{fig:val_2}. The differences between the model's predicted number of DRAM accesses and that from Eyeriss's paper is between 2.18\% and 12.10\%, while the differences between the predicted number of GB accesses and that from Eyeriss's measured results is between -0.70\% and 17.66\%. \hl{The predicted number of DRAM accesses is bigger than that from Eyeriss's measured results because we doesn't consider activation RLC overhead due to the lack of measurement information.} \todor{improve?} \hl{Except CONV1, the differences between the predicted number of GB accesses and that from Eyeriss's measured results is less than 5\%. The stride of CONV1 is 4 which requires reading input activations discontinuously while the input activations are stored sequentially. Therefore, CONV1 has a 17.66\% predictive error.}
% Third, Fig.~\ref{fig:latency} shows that the predicted and Eyeriss's measured latency of executing AlexNet\cite{NIPS2012_4824}'s five CONV layers differ no more than 15.51\%. \hl{The predictive latency is smaller than the measured one. Our prediction assumes an ideal situation where the bandwidth are sufficient while the actual insufficient bandwidth causes stall when processing. } Finally, the predicted throughput is 23.0 GMACS while Eyeriss's measured one is 25.8 GMACS corresponding to a prediction error of less than 11\%. 
% These validation show that our model's predicted performance matches well ($\le $ 17.66\%) with that of chip-measured ones. 

% \todor{analytical model vs. synthesized results of our own design?}

\begin{figure}[!t]
\vspace{-1.2em}
\captionsetup[subfigure]{labelformat=empty}
    \vspace{-1em}
    \centering
    \subfloat{{\includegraphics[width=35mm]{fig/DRAM_new.png} }}\hspace{5pt}
    \subfloat{{\includegraphics[width=35mm]{fig/GB_new.png} }}
    \vspace{-1em}
    \caption{\textbf{The \# of (L) DRAM and (R) GB accesses from Eyeriss~\cite{chen2017eyeriss} and our model for AlexNet's CONV layers.}}
    \vspace{-1.5em}
    \label{fig:val_2}
\end{figure}

\begin{figure}[!b]
   \vspace{-1.5em}
    \centerline{\includegraphics[width=70mm]{fig/latency_big_new.png}}
    \vspace{-1em}
    \caption{\textbf{Comparison on the inference latency from Eyeriss~\cite{chen2017eyeriss} and our model when running AlexNet.}}
    \vspace{-1.5em}
    \label{fig:latency}
\end{figure}

\begin{figure}[h]
    \centerline{\includegraphics[width=75mm]{fig/val_fpga_latency.pdf}}
    \vspace{-1em}
    \caption{\textbf{Our model's predicted latency and the FPGA measured one for the 7 CONV layers of SkyNet~\cite{hao2019fpga}.}}
    \vspace{-1.1em}
    \label{fig:val_fpga}
\end{figure}

\textbf{Validation against Synthesis Results.} Table \ref{fig:val_syn} compares the energy breakdown predicted by our models with that from the synthesis results for AlexNet's CONV3-CONV5 layers when using the proposed SmartExchange accelerator (see Section \ref{sec:Accelerators}). Specifically, the synthesis is performed using a commercial 65nm CMOS technology, where the experiment setting is described in Section \ref{sec:setup}. It can be seen from Table \ref{fig:val_syn} that the difference between our model's predicted energy breakdown differs that from the synthesis results by $\le$5.28\%. 

\ul{In summary}, the aforementioned validation experiments using chip/FPGA-implemented and synthesis results show that our models' predicted performance matches well ($\le $17.66\%) under various experiment settings. 



\begin{table}
\centering
\vspace{3mm}
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}c | ccc c ccc c ccc@{}}\toprule
\multirow{2}{*}{Layer}& \multicolumn{3}{c}{comp. (\%)} & \phantom{x}& \multicolumn{3}{c}{RF(\%)} & \phantom{x}& \multicolumn{3}{c}{GB(\%)}\\ 
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
& Syn. & Pred. & \textbf{$\Delta$} && Syn. & Pred. & \textbf{$\Delta$} && Syn. & Pred. & \textbf{$\Delta$}  \\ 
\midrule
\multirow{1}{*}{CONV3}
$ $ & 38.76 & 34.49 &\textbf{4.26}  && 60.99 & 65.25 & \textbf{4.26} && 0.24 & 0.25 & \textbf{0.01} \\
\midrule
\multirow{1}{*}{CONV4}
$ $ & 39.46 & 34.28 &\textbf{5.19}  && 60.28 & 65.45 & \textbf{5.16} && 0.25 & 0.27 & \textbf{0.02} \\
\midrule
\multirow{1}{*}{CONV5}
$ $ & 31.13 & 25.85 &\textbf{5.28}  && 68.65 & 73.91 & \textbf{5.26} && 0.22 & 0.24 & \textbf{0.02} \\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{\textbf{The energy breakdown from synthesized results and our models for AlexNet's CONV3-CONV5 layers.}}
\label{fig:val_syn}
\vspace{-2em}
\end{table}

==> tex/before-Experiment_Results.tex <==
\section{Experiment Results}\label{sec:before_experiment}
In this section, we present a thorough evaluation of \textit{SmartExchange}, a new algorithm (see Section \ref{sec:algorithm}) and hardware (see Section \ref{sec:Accelerators}) co-design technique. We first introduce the experiment setup and methodology in Section~\ref{sec:setup}, and then compare \textit{SmartExchange}~with state-of-the-art DNN accelerators in terms of the total number of DRAM accesses, energy consumption, and energy-delay product when using representative DNN models and benchmark datasets. Finally, we demonstrate \textit{SmartExchange}'s generalization by showing that when being applied to state-of-the-art DNN accelerators it is consistently able to boost their energy efficiency under various DNN models and hardware configurations.  

\subsection{Experiment Setup and Methodology}\label{sec:setup}

\textbf{Baselines and Methodology. }
Four state-of-the-art accelerators, which uses four representative dataflows, i.e., row stationary (Eyeriss~\cite{eyeriss}), output stationary (ShiDianNao~\cite{du2015shidiannao}), weight stationary (TPU~\cite{jouppi2017datacenter}), and no local reuse (DianNao~\cite{chen2014diannao}) as listed Table~\ref{table:dataflows}, are considered in our experiments. \ul{First}, we consider the peak performance between the proposed \textit{SmartExchange} accelerator and the baselines using the reported data in their papers. \ul{Second},
we further evaluate our \textit{SmartExchange} accelerator against these competitive baselines on various DNNs and datasets. For this second set of experiments, we perform design space exploration using the proposed analytical models (see Section~\ref{sec:Framework}) to further optimize both the ordering and tiling factors of each baseline in order to boost their energy efficiency and reduce their latency, targeting a more solid evaluation. 

\textbf{Benchmarks.}
We use four representative DNNs (including \ul{VGG19}\footnotemark[\value{footnote}], \ul{AlexNet}\cite{NIPS2012_4824}, \ul{VGG16}\cite{simonyan2014very}, and \ul{ResNet50}\cite{he2016deep}) and two benchmark datasets (\ul{CIFAR-10 (C10)} \cite{cifar10} and \ul{ImageNet (IN)} \cite{Deng09imagenet}). Regarding the precision, we adopt \emph{(i)} 8-bit inputs/activations for both the original and \textit{SmartExchange}-based DNNs; and \emph{(ii)} 8-bit weights for the original DNNs, and 8-bit/4-bit precision for the basis and coefficient matrices, respectively, in the \textit{SmartExchange}-based DNNs.

\textbf{Technology-dependent Parameters.} 
\begin{comment}
Regarding the tech\-nology-dependent unit energy/delay, we mainly refer to~\cite{yang2018dnn} which characterizes unit energy/delay based on post-layout simulations using a commercial 28nm CMOS technology. Specifically, we use \emph{(i)} a state-of-the-art tool in~\cite{tangmlpat} which uses the methodology of CACTI 6.0~\cite{muralimanohar2007optimizing} to estimate the unit energy cost of GB accesses and NoC accesses; and \emph{(ii)} refer to~\cite{yang2018dnn} for the unit energy cost of RF accesses under various memory sizes and MAC operations.
Table~\ref{table:unit_energy} list the unit energy costs per 16-bit when accessing various memories with different storage sizes, which are used in our performance evaluation. 

We adopt a frequency of 400MHz, as ~\cite{yang2018dnn} validated that a frequency of 400MHz or less leads to zero timing violations using post-layout simulations and accelerators with various dataflows (e.g., output stationary and weight stationary) using representative DNN models~\cite{NIPS2012_4824, howard2017mobilenets, szegedy2015going} on ImageNet.
To be conservative, we adopt the energy of a MAC operation to estimate the energy cost of restoring weights (i.e., three shift and two addition operations).
\end{comment}
% \hl{Need to update} 
For benchmarking \textit{SmartExchange}'s peak energy efficiency and throughput (see Table \ref{table:comparison}) over state-of-the-art accelerators, we synthesize the RTL implementation of \textit{SmartExchange} based on a commercial 65nm CMOS technology using the Synopsys Design and Arm Artisan Memory Compilers. The resulting performance of the unit energies and \textit{SmartExchange} are listed in Table \ref{table:unit_energy} and Table \ref{table:comparison}, respectively. We obtain the unit energy costs following a state-of-the-art method in~\cite{yang2018dnn}. Specifically, proper testbenches are set at the input/output ports of the memory/computation units, and the energy is calculated using the tool of PrimeTime PX~\cite{PTPX} based gate-level netlists, where the switching activities are obtained in the simulations. We refer to ~\cite{yang2018dnn} for the unit energy of DRAM access, which is 
200pJ per 8-bit.

% from PT with proper testbench/switching activities

% Additionally, we use single-port SRAMs in our design. 

% Regarding the technology-dependent unit energy/delay, we synthesize the RTL code into a commercial 65nm CMOS technology using Synopsys Design Compiler and synthesize the memory into the 28nm technology using Arm Artisan Memory Compiler. All of our RTL designs achieve 1GHz operation with no timing violations. To get the unit energy costs, the proper testbenches is set on the ports and the propagated through the gate-level netlist in Prime Time PX. \todob{e.g., the RE works every cycle. }
% Our energy ratios between memory and MAC are smaller than those reported in Eyeriss~\cite{eyeriss}. There are several possible reasons: we use 28nm technology instead of 65nm; our MAC includes the DFFs; the memory is set to the largest port width; we use single-port SRAM instead of dual-port SRAM in Eyeriss.  \todob{needed?} 

% \vspace{-0.8em}
% \begin{table}[!hbtp]
% \small
% \centering
% \renewcommand\arraystretch{1}
% \setlength{\tabcolsep}{5pt}

%         \begin{minipage}{.5\linewidth}
%         %   \caption{}
%           \centering
%             \begin{tabular}{@{}c c@{}}\toprule
%             	\textbf{RF size} & \textbf{Energy (pJ)} \\
%             	\midrule
%             % 	128B & 0.342\\
%             % 	256B & 0.349\\
%             % 	1KB & 0.373\\
%             % 	4KB & 0.445\\
%             	0.5KB & 0.889\\
%             	1KB & 0.920\\
%             	2KB & 1.004\\
%             	4KB & 1.454\\
%             	%64B & 0.12\\
%             	%128B & 0.24\\
%             	%256B & 0.48\\
%             	%512B & 0.96\\
%             	%1024B & 1.92\\
%             	\midrule
%             % 	MAC & 0.426 \\
%                 MAC & 0.363 \\
%             	\midrule 
%             % 	rebuilding & 0.222 \\ 
%                 rebuilding &  0.132\\ 
%             	%\midrule 
%             	%NoC & 2.768\\
%             	%\midrule
%             	%DRAM & 200 \\
%                 \bottomrule
%                 \end{tabular}
%         \end{minipage}%
%         \begin{minipage}{.5\linewidth}
%           \centering
%             % \caption{}
%             \begin{tabular}{@{}c c@{}}\toprule
%             	\textbf{SRAM size} & \textbf{Energy (pJ)} \\
%             	\midrule
%             % 	1KB & 3.141 \\
%             % 	2KB & 3.546 \\
%             % 	16KB & 5.952 \\
%             % 	64KB & 10.191 \\
%             % 	128KB & 13.119 \\
%             % 	256KB &  16.420 \\
%                 0.5KB & 3.71\\
%                 1KB & 3.78 \\
%             	2KB & 3.91 \\
%             	4KB & 3.99\\
%             	8KB & 4.45\\
%             % 	16KB & 2.07 \\
%             % 	64KB & 10.191 \\
%             % 	128KB & 13.119 \\
%             % 	256KB &  16.420 \\
%             	%\midrule 
%             	%NoC & 2.768\\
%             	\midrule
%             	DRAM & 200 \\
%                 \bottomrule
%                 \end{tabular}
%         \end{minipage} 
%         \vspace{-0.8em}
%     \caption{\textbf{Unit energy costs per 8-bit corresponding to various memory accesses and computations based on synthesis results from a commercial 65nm CMOS technology.}}
%     \vspace{-1em}
%     \label{table:unit_energy}
% \end{table}

\begin{table}
\small
\centering
\caption{Unit energy costs per 8-bit corresponding to various memory accesses and computations based on synthesis results from a commercial 65nm CMOS technology.}
% \setlength\tabcolsep{0pt}
\ra{1.3}
\begin{tabular}{@{}c || c| c c c c c @{}}\toprule
\textbf{MAC} &\multirow{2}{*}{\textbf{RF}}
& \textbf{size} & 0.5K & 1KB & 2KB & 4KB \\ \cline{3-7}
1.60 pJ & & \textbf{E. (pJ)} & 0.89 & 0.92 & 1.00 & 1.45\\
\midrule
\textbf{RE} & \multirow{2}{*}{\textbf{SRAM}}
& \textbf{size} & 1KB & 2KB & 4KB & 8KB \\ \cline{3-7}
0.97 pJ & & \textbf{E. (pJ)} & 3.78 & 3.91 & 3.99 & 4.45 \\
\bottomrule
\end{tabular}
    \label{table:unit_energy}
\end{table}

% \begin{table}
% \centering
% \caption{Benefits of distributed local analog buffers}
% \vspace{3mm}
% \small
% % \setlength\tabcolsep{0pt}

% \begin{tabular}{@{}c| c c c c c c c c@{}}\toprule
% \multirow{2}{*}{RF}
% % & \textbf{RF size} & 128B & 256B & 1KB & 4KB & \\\cline{2-7}
% & \textbf{RF size} & \multicolumn{5}{c}{\begin{tabular}{cccc} 128B & 256B & 1KB & 4KB \end{tabular}} & \multirow{2}{*}{X} & \multirow{2}{*}{X}  \\ \cline{2-7}
% & \textbf{Energy (pJ)} & \multicolumn{5}{c}{\begin{tabular}{cccc} 0.34 & 0.35 & 0.37 & 0.45 \end{tabular}}   \\ 
% % & \textbf{Energy (pJ)} & 0.34 & 0.35 & 0.37 & 0.45 &   \\ 
% \midrule
% \multirow{2}{*}{SRAM} 
% & \textbf{SRAM size} & 1KB & 2KB & 4KB & 8KB & 16KB & \multirow{2}{*}{X} & \multirow{2}{*}{X}\\\cline{2-7}
% & \textbf{Energy (pJ)} & 1.27 & 1.40 & 1.64 & 1.77 & 2.07   \\ 

% \bottomrule
% \end{tabular}
% \end{table}

% %\vspace{-1em}
% \begin{table}[!hbtp]
% \small
% \centering
% \renewcommand\arraystretch{1}
% \setlength{\tabcolsep}{5pt}

%         \begin{minipage}{.5\linewidth}
%         %   \caption{}
%           \centering
%             \begin{tabular}{@{}c c@{}}\toprule
%             	\textbf{RF size} & \textbf{Energy (pJ)} \\
%             	\midrule
%             	16B & 0.03\\
%             	32B & 0.06\\
%             	%64B & 0.12\\
%             	%128B & 0.24\\
%             	256B & 0.48\\
%             	%512B & 0.96\\
%             	1024B & 1.92\\
%             	\midrule
%             	MAC & 0.075 \\
%             	\midrule 
%             	rebuilding & 0.075 \\ 
%             	%\midrule 
%             	%NoC & 2.768\\
%             	%\midrule
%             	%DRAM & 200 \\
%                 \bottomrule
%                 \end{tabular}
%         \end{minipage}%
%         \begin{minipage}{.5\linewidth}
%           \centering
%             % \caption{}
%             \begin{tabular}{@{}c c@{}}\toprule
%             	\textbf{SRAM size} & \textbf{Energy (pJ)} \\
%             	\midrule
%             	1KB & 3.141 \\
%             	2KB & 3.546 \\
%             	16KB & 5.952 \\
%             	64KB & 10.191 \\
%             	128KB & 13.119 \\
%             	256KB &  16.420 \\
%             	\midrule 
%             	NoC & 2.768\\
%             	\midrule
%             	DRAM & 200 \\
%                 \bottomrule
%                 \end{tabular}
%         \end{minipage} 
%         \vspace{-0.8em}
%     \caption{\textbf{Unit energy costs per 16-bit when accessing various memory hierarchies with different sizes\cite{muralimanohar2007optimizing,tangmlpat,yang2018dnn}.} \todor{using our own technology}}
%             %\vspace{-1em}-1.5    
%     \label{table:unit_energy}
% \end{table}


\subsection{SmartExchange vs. Pior Arts }\label{sec:dedicated}

\begin{scriptsize}
\begin{table}[h!]
\caption{Peak energy efficiency and throughput of \textit{SmartExchange} and state-of-the-art DNN accelerators including Eyeriss~\cite{chen2017eyeriss}, ShiDianNao~\cite{du2015shidiannao}, and DianNao~\cite{chen2014diannao}. }
\centering
\scriptsize
\begin{tabular}{|p{1.2cm}<{\centering}|p{0.5cm}<{\centering}|p{0.58cm}<{\centering}|p{0.6cm}<{\centering}|p{1.1cm}<{\centering}|p{0.6cm}<{\centering}|p{1.2cm}<{\centering}|}
\hline
~ & \multirow{2}{*}{\textbf{Tech.}} & \multirow{2}{*}{\textbf{Freq.}} & \multicolumn{2}{c|}{\textbf{Throughput}} & \multicolumn{2}{c|}{\textbf{Energy Efficiency}} \\1`
~ & \multirow{2}{*}{\textbf{($nm$)}} & \multirow{2}{*}{\textbf{($MHz$)}} & \multicolumn{2}{c|}{\textbf{($GOP/s$)}} & \multicolumn{2}{c|}{\textbf{($GOPs/W$)}} \\\cline{4-7}

~ & ~ & ~ & Theo.$^+$ & Model$^*$ & Theo.$^+$ & Model$^*$\\

\hline
\hline
Eyeriss &  65 & 250 & 84 & 27$^{VGG16-IN}$ & -- & 115$^{VGG16-IN}$\\
\hline
ShiDianNao & 65 & 1000 & 128 & -- & \multicolumn{2}{c|}{400$^{CONV~of~LeNet}$} \\
\hline
DianNao & 65 & 980 & 452 & -- & 931 & -- \\
\hline
Ours & 65 & 1000 & 512 & 361$^{VGG16-IN}$ & -- & 1016$^{VGG16-IN}$ \\
%Ours & 65$^+$ & 172 & 88.1 & 99.3$^c$ & -- & 541$^c$ \\
\hline
\end{tabular}
\\
\begin{tablenotes}
\item{$^+$ Theoretical peak performance of 100\% PE utilization.}
\item{$^*$ Performance of actually running DNNs where PE <100\%.}
%\item{$^a$ VGG16-IN~\cite{simonyan2014very} batch size=3~\cite{chen2017eyeriss} }
%\item{$^b$ Power of running CONV layers only~\cite{du2015shidiannao} divided by peak throughput}
%\item{$^+$ Scaled up to 65nm}
%\item{$^c$ VGG16-IN~\cite{simonyan2014very}, equivalent performance considering input and coefficient sparsity}
\end{tablenotes}
\label{table:comparison}
\end{table}
\end{scriptsize}


\textbf{Overall Peak Performance.}
% We next compare our proposed dedicated accelerator that is designed to take advantage of the SED algorithm with four state-of-the-art accelerators. 
\ul{For this experiments}, we compare the peak energy efficiency and throughput of \textit{SmartExchange} and state-of-the-art DNN accelerators including Eyeriss~\cite{chen2017eyeriss}, ShiDianNao~\cite{du2015shidiannao}, and DianNao~\cite{chen2014diannao}. Table~\ref{table:comparison} summarizes the comparison results, where the baselines' performance are from those reported in their papers. We can see that our \textit{SmartExchange} accelerator has $13.37\times$ higher throughput and is $8.83\times$ more energy efficient than Eyeriss when running VGG16 \cite{simonyan2014very} using the ImageNet dataset. Compared with the theoretical performance of ShiDianNao, our proposed accelerator has $2.82\times$ higher throughput, and is $2.54\times$ more energy efficient. Note that the higher throughput of DianNao is obtained assuming a 100\% PE utilization, which is in general not possible in practice and results in impractically higher inference frequency and thus throughput. Our \textit{SmartExchange} accelerator still achieves $1.09\times$ higher energy efficiency than DianNao. Note that TPU is not considered here as it is dedicated for data center applications.

\ul{For the remaining experiments} in this section, we compare the proposed \textit{SmartExchange} accelerator with the four state-of-the-art DNN accelerators in terms of the total number of DRAM accesses, energy consumption, and energy-delay product when using representative DNN models and benchmark datasets. To do so, we use our proposed modeling framework (see Section~\ref{sec:Framework}) to first optimize and then evaluate the performance of both the baseline and our proposed accelerators. 
For practical deployment, \emph{(i)} all the accelerators are optimized subjecting to a hard constraint on both the number of PEs and maximum memory area (referring to \cite{eyeriss}) for each data type; and \emph{(ii)} in the optimization process we also make use of the input sparsity for reducing associated energy costs of both data movements and computations. 
% \todor{An example to show the optimized dataflow?}

Considering the large design space of DNN accelerators,
it is not surprising to \textbf{consistently} observe that the performance of the resulting optimal designs for the baselines \textbf{even outperforms their self-reported ones}, which are mostly hand crafted dedicated designs by domain experts.

\begin{figure}[!t]
    \centerline{\includegraphics[width=70mm]{fig/dram_accesses_mark_2.png}}
    \caption{\ul{The total number of DRAM accesses} of the \textit{SmartExchange} and state-of-the-art accelerators with various dataflows using four representative DNN models and two benchmark datasets, where VGG19-C10 denotes the combination of VGG19 and CIFAR-10.}
    \label{fig:DRAM_1}
\end{figure}

\textbf{DRAM Accesses.} 
The energy cost of DRAM accesses can be two orders of magnitude higher than that of dot product computation \cite{eyeriss}. For this experiment, we perform optimization to minimize the number of DRAM accesses for both the \textit{SmartExchange} and baseline accelerators by ensuring that partial sums of the  activations are not written back to the off-chip DRAM unless the final activations are obtained or the on-chip GB reaches its full capacity. \ul{Fig.}~\ref{fig:DRAM_1} shows the total number of DRAM accesses (in terms of the total number of bits) per operation considering all three data types (i.e., weights, inputs/outputs) for both our proposed accelerator (depicted as ``proposed'' ) and the four baselines when running various DNNs on the two datasets. We can see that our \textit{SmartExchange} accelerator consistently outperforms all the four baselines under all the considered DNN models and datasets, and achieves a reduction on the total number of DRAM accesses ranging from \textbf{$\boldsymbol{1.5 \times}$ to $\boldsymbol{9.8 \times}$}, demonstrating the effectiveness of \textit{SmartExchange}'s algorithm-hardware co-design effort in reducing the high-cost DRAM accesses. As these DNN models have different depth and layer structure that corresponds to different computation and movement patterns, the much reduced number of required DRAM accesses validate that \textit{SmartExchange} accelerators' effectiveness in reducing the data movements \textbf{is generalizable to varied DNNs}.

\begin{figure}[!b]
    \centerline{\includegraphics[width=70mm]{fig/norm_energy_new.png}}
    \caption{\ul{The normalized  energy consumption} of the \textit{SmartExchange} and state-of-the-art accelerators with various dataflows using four representative DNN models and two benchmark datasets, where VGG16-IN \cite{simonyan2014very} denotes the combination of VGG16 \cite{simonyan2014very} and ImageNet \cite{Deng09imagenet}.}
    \label{fig:energy_1}
\end{figure}

\textbf{Energy Consumption.} 
\ul{Fig.}~\ref{fig:energy_1} shows the normalized energy consumption of the \textit{SmartExchange} and baseline accelerators using four DNN models and two benchmark datasets. It is shown that \textit{SmartExchange} accelerator consumes the least energy under all the considered DNN models and datasets, achieving a reduction on the energy cost ranging from \textbf{$\boldsymbol{1.5 \times}$ to $\boldsymbol{4.9 \times}$}. The \textit{SmartExchange} accelerator's outstanding energy efficiency performance is a result of \textit{SmartExchange}'s algorithm hardware co-design effort to effectively trade the much higher cost memory storage/accesses for the lower cost computations (e.g., rebuilding the weights using the basis and coefficient matrices at the least costly RF and PE levels). Again, we observe that \textit{SmartExchange} outperforms all the baselines using various DNN models and datasets. 

\textbf{Energy Delay Product.} 
\ul{Fig.}~\ref{fig:EDP_1} shows that our proposed \textit{SmartExchange} accelerator achieves the best EDP performance among all the accelerators under all considered DNN models and datasets. Specifically, the \textit{SmartExchange} accelerator reduces the EDP by \textbf{$\boldsymbol{1.6 \times}$ to $\boldsymbol{9.6 \times}$}. Note that we do not consider the case when using VGG19 \footnotemark[\value{footnote}] and CIFAR-10\cite{cifar10} dataset as the corresponding EDP of the baseline ShiDianNao is very high due to the fact that the output feature size in VGG19-C10 \footnotemark[\value{footnote}] (thus the corresponding number of active PEs) is very small, whereas the output channels is relatively much larger, leading to a much increased inference latency as ShiDianNao was designed to handle small-scale DNNs (e.g., LeNet-5).  
Besides, the EDP improvement achieved by the \textit{SmartExchange} accelerator is consistently higher than its energy efficiency improvement (see Fig.~\ref{fig:energy_1}) under the same condition (e.g., the same accelerator design, DNN models, and datasets), demonstrating that our \textit{SmartExchange} accelerator also leads to a smaller latency than all the baselines.

\begin{figure}[!t]
    \centerline{\includegraphics[width=75mm]{fig/norm_EDP_new_NA.png}}
    \caption{\ul{The normalized energy-delay product} of the \textit{SmartExchange} and state-of-the-art accelerators with various dataflows using four representative DNN models and two datasets, where ResNet50-IN \cite{he2016deep} denotes the combination of ResNet50 \cite{he2016deep} and ImageNet \cite{Deng09imagenet}.}
    \label{fig:EDP_1}
\end{figure}

% \textbf{Benefits of Coefficient Sparsity.} 
% Even though the \textit{SmartExchange} accelerator can leverage the enforced sparsity of the coefficient matrices (see Section \ref{sec:algorithm}), e.g., $15.71\% \sim 56.14\%$ among the four DNN models and two datasets, for improved performance, we do not consider this sparsity in the aforementioned experiments for a conservative evaluation of the \textit{SmartExchange} idea. In this experiment, we compare the energy consumption of the \textit{SmartExchange} accelerator when considering the coefficients' sparsity with that of the \textit{SmartExchange} accelerator without making use of this sparsity. Specifically, the former is \textbf{50.4\%, 44.4\%, 58.5\%, and 54.4\%} more energy efficient, respectively, on the benchmark settings of VGG19-C10\footnotemark[\value{footnote}], AlexNet-IN\cite{NIPS2012_4824}, VGG16-IN\cite{simonyan2014very}, and ResNet50-IN\cite{he2016deep}, leading to a geometric mean of 51.6\%. 


\begin{comment}
\subsection{Generalization of SmartExchange}\label{sec:Baselines+SE}
As discussed in Section~\ref{sec:Existing_accelerators}, the proposed \textit{SmartExchange} idea is a generic algorithm hardware co-design technique that can be generalized to state-of-the-art accelerator for further boosting their energy efficiency. In this experiment, we evaluates the \textit{SmartExchange}-boosted baseline accelerators (see Section~\ref{sec:Existing_accelerators}) to validate the generality of \textit{SmartExchange}.
\ul{Fig.}~\ref{fig:energy_3} shows that the normalized energy consumption of the \textit{SmartExchange}-boosted accelerators is consistently smaller than that of the corresponding original accelerators, with a reduction ranging from $1.04\times$ to $1.59\times$. We observe that DianNao has the highest boosted improvement of $1.42\times$ to $1.59\times$ in all considered DNNs and datasets, as DianNao's energy cost is dominated by the DRAM accesses while the \textit{SmartExchange} algorithm via SED can aggressively reduce the data movements associated with the DRAM. In addition, even for the TPU accelerator which is dedicated to maximize weight reuses, the \textit{SmartExchange}-boosted accelerators can still achieve a $1.28\times$ to $1.38\times$ reduction. These results demonstrate and validate \textit{SmartExchange}'s generalization.
\end{comment}

